ALIGN-MLM: Word Embedding Alignment is Crucial for Multilingual Pre-training

Multilingual pre-trained models exhibit zero-shot cross-lingual transfer, where a model fine-tuned on a source language achieves surprisingly good performance on a target language. While studies have attempted to understand transfer, they focus only on MLM, and the large number of differences between natural languages makes it hard to disentangle the importance of different properties. In this work, we specifically highlight the importance of word embedding alignment by proposing a pre-training objective (ALIGN-MLM) whose auxiliary loss guides similar words in different languages to have similar word embeddings. ALIGN-MLM either outperforms or matches three widely adopted objectives (MLM, XLM, DICT-MLM) when we evaluate transfer between pairs of natural languages and their counterparts created by systematically modifying specific properties like the script. In particular, ALIGN-MLM outperforms XLM and MLM by 35 and 30 F1 points on POS-tagging for transfer between languages that differ both in their script and word order (left-to-right v.s. right-to-left). We also show a strong correlation between alignment and transfer for all objectives (e.g., rho=0.727 for XNLI), which together with ALIGN-MLM's strong performance calls for explicitly aligning word embeddings for multilingual models.

==> Figures_and_Tables/dump.tex <==
\begin{table*}[ht]
\centering
% Uncomment to resize
\resizebox{2\columnwidth}{!}{
\begin{tabular}{clccccccccc}
\toprule
\multicolumn{1}{c}{\bf{Pre-training method}} & \bf{Transformation} & \multicolumn{3}{c}{\bf{XNLI}}                                                                                                    & \multicolumn{3}{c}{\bf{NER}}                                                                                                     & \multicolumn{3}{c}{\bf{POS}}                                                                                                     \\ \cmidrule(){3-5} \cmidrule(){6-8} \cmidrule(){9-11}
\multicolumn{1}{c}{}                    &                & \bs{} & \bz{} & BZ-BS & \bs{} & \multicolumn{1}{c}{BZ} & \multicolumn{1}{c}{BZ-BS} & \multicolumn{1}{c}{BS} & \multicolumn{1}{c}{BZ} & \multicolumn{1}{c}{BZ-BS} \\ \midrule
                                        & Trans          & 76.4                                           & 74.9                                           & -1.5                                              & 80.6                                           & 78.0                                           & -2.6                                              & 95.0                                           & 94.6                                           & -0.4                                              \\
                                        & Trans + Inv    & 73.9                                           & 56.7                                           & -17.2                                             & 79.2                                           & 35.9                                           & -43.3                                             & 95.0                                           & 56.5                                           & -38.5                                             \\
\multirow{-3}{*}{MLM}                   & Trans + Syn    & 73.5                                           & 69.0                                           & -4.5                                              & 71.3                                           & 52.3                                           & -19.0                                             & 93.6                                           & 91.6                                           & -2.0                                              \\ \midrule
                                        & Trans          & 77.3                                           & 77.5                                           & 0.2                                               & 80.8                                           & 79.7                                           & -1.1                                              & 95.0                                           & 94.8                                           & -0.2                                              \\
                                        & Trans + Inv    & 75.4                                           & 67.2                                           & -8.2                                              & 80.0                                           & 60.7                                           & -19.4                                             & 95.0                                           & 61.8                                           & -33.2                                             \\
\multirow{-3}{*}{XLM}                   & Trans + Syn    & 76.1                                           & 74.1                                           & -1.9                                              & 71.5                                           & 59.6                                           & -11.9                                             & 93.7                                           & 92.7                                           & -0.9                                              \\ \midrule
                                        & Trans          & 77.0                                           & 75.9                                           & -1.1                                              & 79.3                                           & 78.3                                           & -1.1                                              & 95.1                                           & 94.8                                           & -0.3                                              \\
                                        & Trans + Inv    & 74.5                                           & 65.3                                           & -9.2                                              & 79.1                                           & 59.8                                           & -19.3                                             & 95.0                                           & 76.0                                           & -19.0                                             \\
\multirow{-3}{*}{Dict-MLM}              & Trans + Syn    & 74.3                                           & 72.2                                           & -2.2                                              & 71.4                                           & 57.6                                           & -13.8                                             & 93.6                                           & 92.6                                           & -1.0                                              \\ \midrule
                                        & Trans          & 75.1                                           & 75.5                                           & 0.5                                               & 79.4                                           & 78.6                                           & -0.8                                              & 94.9                                           & 94.8                                           & -0.1                                              \\
                                        & Trans + Inv    & 75.5                                           & 68.8                                           & -6.7                                              & 80.0                                           & 64.5                                           & -15.5                                             & 95.0                                           & 92.0                                           & -3.0                                              \\
\multirow{-3}{*}{Aligned-MLM}           & Trans + Syn    & 74.7                                           & 71.1                                           & -3.6                                              & 71.3                                           & 58.3                                           & -13.1                                             & 93.7                                           & 92.9                                           & -0.8                                              \\ \bottomrule
\end{tabular}
% Uncomment for resize
}
\end{table*}

==> Figures_and_Tables/old_hyperparameters.tex <==
\begin{table} 
	\centering
	\begin{tabular}{ |p{8cm}|p{4cm}|  }
		\hline
		\multicolumn{2}{|c|}{Model Parameters (standard for RoBERTa model)} \\
		\hline
		Parameter Name& Parameter Value \\
		\hline
		Model Type & RoBERTa\\
		Attention Dropout Rate & 0.1 \\
		Hidden Activation Function & GELU\\
		Hidden Dropout Probability & 0.1\\
		Hidden Size\tablefootnote{During finetuning, the hidden size is 128} &512\\
		Intermediate Size & 2048 \\
		Layer Norm Epsilon & $10^{-5}$ \\
		Position Embeddings per Instance & 512 \\
		Number of Attention Heads & 8\\
		Number of Hidden Layers & 8\\
		Type Vocab Size & 2\\
		Number of Languages\tablefootnote{We only train on two languages at a time.} & 2\\
		Vocab Size\tablefootnote{This is for one language. When the transliteration transformation is used, the vocab size is doubled.} & 40000\\
		Learning Rate\tablefootnote{The learning rate starts at 0, increases to a max of $10^{-4}$ linearly, then drops linearly to 0} & $10^{-4}$\\
		Training Steps & 500000\\
		\hline
	\end{tabular}
\caption{Hyperparameters used for pretraining.}
\label{app:tab:}
\end{table}

==> Figures_and_Tables/other_tables.tex <==



% \begin{table*}[ht]
% \centering
% % Uncomment to resize
% \resizebox{2\columnwidth}{!}{
% \begin{tabular}{clrrrrrrrrr}
% \toprule
% \multicolumn{1}{l}{\bf{Varying TLM Data}} & \bf{Transformation} & \multicolumn{2}{c}{\bf{XNLI}} & \multicolumn{2}{c}{\bf{NER}} & \multicolumn{2}{c}{\bf{POS}} \\
% \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}
% \multicolumn{1}{l}{} & & \multicolumn{1}{l}{BZ} & \multicolumn{1}{l}{BS-BZ} & \multicolumn{1}{l}{BZ} & \multicolumn{1}{l}{BS-BZ} & \multicolumn{1}{l}{BZ} & \multicolumn{1}{l}{BS-BZ} \\ 
% \midrule
% 1\% & Trans + Inv & 59.8                   & 16.1                      & 40.2                   & 39.5                      & 66.9                   & 28.1                      \\
% \midrule
% 10\% & Trans + Inv & 65.8                   & 9.5                       & 59.4                   & 20.3                    & 63.6                   & 31.5                      \\ 
% \midrule
% 25\% & Trans + Inv & 67.2                   & 8.2                       & 60.7                   & 19.4                    & 61.8                   & 33.2                      \\
% \midrule
% 100\% & Trans + Inv & 65.2                   & 9.8                       & 62.4                   & 17.6                    & 60.0                   & 35.1                      \\
% \bottomrule
% \end{tabular}
% % Uncomment for resize
% }
% \end{table*}

% \begin{table*}[ht]
% \centering
% % Uncomment to resize
% \resizebox{2\columnwidth}{!}{
% \begin{tabular}{clrrrrrrrrr}
% \toprule
% \multicolumn{1}{l}{\bf{Percentage Shared}} & \bf{Transformation} & \multicolumn{2}{c}{\bf{XNLI}} & \multicolumn{2}{c}{\bf{NER}} & \multicolumn{2}{c}{\bf{POS}} \\
% \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}
% \multicolumn{1}{l}{} & & \multicolumn{1}{l}{BZ} & \multicolumn{1}{l}{BS-BZ} & \multicolumn{1}{l}{BZ} & \multicolumn{1}{l}{BS-BZ} & \multicolumn{1}{l}{BZ} & \multicolumn{1}{l}{BS-BZ} \\ 
% \midrule
% 0\% & Trans + Inv & 67.2 & 8.2 & 60.7 & 19.4 & 61.8 & 33.2  \\
% \midrule
% 25\% & Trans + Inv & 71.3 & 5.2   & 64.0 & 15.8  & 92.6 & 2.4   \\
% \midrule
% 50\% & Trans + Inv & 72.2 & 2.8   & 42.5 & 37.5  & 94.4 & 0.6   \\
% \bottomrule
% \end{tabular}
% % Uncomment for resize
% }
% \end{table*}

% \begin{table*}[ht]
% \centering
% % Uncomment to resize
% \resizebox{2\columnwidth}{!}{
% \begin{tabular}{clrrrrrrrrr}
% \toprule
% \multicolumn{1}{c}{\bf{\% Tokens in}} & \bf{Transformation} & \multicolumn{3}{c}{\bf{XNLI}}                                                                                                    & \multicolumn{3}{c}{\bf{NER}}                                                                                                     & \multicolumn{3}{c}{\bf{POS}}                                                                                                     \\ \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}
% \multicolumn{1}{c}{\bf{Bilingual Dictionary}}                    &                & \multicolumn{1}{l}{BS} & \multicolumn{1}{l}{BZ} & \multicolumn{1}{l}{BS-BZ} & \multicolumn{1}{l}{BS} & \multicolumn{1}{l}{BZ} & \multicolumn{1}{l}{BS-BZ} & \multicolumn{1}{l}{BS} & \multicolumn{1}{l}{BZ} & \multicolumn{1}{l}{BS-BZ} \\ \midrule
% & Trans          & 76.4                     & 74.9                   & 1.5                       & 80.6                    & 78.0                   & 2.6                       & 95.0                    & 94.6                   & 0.4                       \\
%                                & Trans + Inv    & 73.9                     & 56.7                   & 17.2                      & 79.2                    & 35.9                   & 43.3                      & 95.0                    & 56.5                   & 38.5                      \\
% \multirow{-3}{*}{0\%}                   & Trans + Syn    & 73.5                     & 69.0                   & 4.5                       & 71.3                    & 52.3                   & 19.0                      & 93.6                    & 91.6                   & 2.0                       \\
% \midrule
%                                & Trans          & 75.1                     & 75.5                   & -0.5                      & 79.4                    & 78.6                   & 0.8                       & 94.9                    & 94.8                   & 0.1                       \\
%                                & Trans + Inv    & 75.5                     & 68.8                   & 6.7                       & 80.0                    & 64.5                   & 15.5                      & 95.0                    & 92.0                   & 3.0                       \\
% \multirow{-3}{*}{25\%}                   & Trans + Syn    & 74.7                     & 71.1                   & 3.6                       & 71.3                    & 58.3                   & 13.1                      & 93.7                    & 92.9                   & 0.8                       \\
% \midrule
%                                & Trans          & 75.3                     & 74.6                   & 0.7                       & 80.4                    & 79.1                   & 1.3                       & 95.0                    & 94.9                   & 0.1                       \\
%                                & Trans + Inv    & 74.4                     & 68.7                   & 5.7                       & 79.7                    & 65.7                   & 14.0                      & 95.0                    & 93.5                   & 1.5                       \\
% \multirow{-3}{*}{50\%}                   & Trans + Syn    & 73.8                     & 72.2                   & 1.6                       & 71.8                    & 60.3                   & 11.5                      & 93.5                    & 92.8                   & 0.7                       \\
% \midrule
%                                & Trans          & 75.7                     & 75.1                   & 0.6                       & 79.8                    & 78.8                   & 1.0                       & 95.0                    & 94.9                   & 0.1                       \\
%                                & Trans + Inv    & 73.6                     & 70.1                   & 3.5                       & 79.4                    & 45.5                   & 33.8                      & 95.0                    & 93.7                   & 1.3                       \\
% \multirow{-3}{*}{100\%}                   & Trans + Syn    & 74.9                     & 73.4                   & 1.6                       & 71.4                    & 60.3                   & 11.2                      & 93.7                    & 93.1                   & 0.6 \\
% \bottomrule
% \end{tabular}
% % Uncomment for resize
% }
% \caption{Performance of \dict{} when varying the percentage of tokens in the bilingual dictionary between \lang1 and \lang2.}
% \end{table*}


% \begin{table*}[ht]
% \centering
% % Uncomment to resize
% \resizebox{2\columnwidth}{!}{
% \begin{tabular}{clrrrrrrrrr}
% \toprule
% \multicolumn{1}{c}{\bf{\% Tokens in}} & \bf{Transformation} & \multicolumn{3}{c}{\bf{XNLI}}                                                                                                    & \multicolumn{3}{c}{\bf{NER}}                                                                                                     & \multicolumn{3}{c}{\bf{POS}}                                                                                                     \\ \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}
% \multicolumn{1}{c}{Bilingual Dictionary}                    &                & \multicolumn{1}{l}{BS} & \multicolumn{1}{l}{BZ} & \multicolumn{1}{l}{BS-BZ} & \multicolumn{1}{l}{BS} & \multicolumn{1}{l}{BZ} & \multicolumn{1}{l}{BS-BZ} & \multicolumn{1}{l}{BS} & \multicolumn{1}{l}{BZ} & \multicolumn{1}{l}{BS-BZ} \\ \midrule
%  & Trans          & 77.0                     & 75.9                   & 1.1                       & 79.3                    & 78.3                   & 1.1                       & 95.1                    & 94.8                   & 0.3                       \\
%                                & Trans + Inv    & 74.5                     & 65.3                   & 9.2                       & 79.1                    & 59.8                   & 19.3                      & 95.0                    & 76.0                   & 19.0                      \\
% \multirow{-3}{*}{25\%}                               & Trans + Syn    & 74.3                     & 72.2                   & 2.2                       & 71.4                    & 57.6                   & 13.8                      & 93.6                    & 92.6                   & 1.0                       \\
% \midrule
% & Trans          & 76.8                     & 76.6                   & 0.2                       & 79.7                    & 79.2                   & 0.5                       & 95.1                    & 94.8                   & 0.2                       \\
%                                & Trans + Inv    & 75.5                     & 69.4                   & 6.0                       & 79.4                    & 63.4                   & 15.9                      & 94.9                    & 91.5                   & 3.4                       \\
% \multirow{-3}{*}{50\%}                               & Trans + Syn    & 73.7                     & 70.8                   & 2.9                       & 71.7                    & 58.3                   & 13.4                      & 93.6                    & 92.7                   & 0.9                       \\
% \midrule
% & Trans          & 77.2                     & 76.5                   & 0.8                       & 79.8                    & 78.7                   & 1.1                       & 95.0                    & 94.8                   & 0.2                       \\
%                                & Trans + Inv    & 74.1                     & 70.6                   & 3.4                       & 78.9                    & 56.5                   & 22.4                      & 95.0                    & 94.1                   & 0.8                       \\
% \multirow{-3}{*}{100\%}                               & Trans + Syn    & 74.6                     & 74.0                   & 0.6                       & 71.2                    & 58.2                   & 13.0                      & 93.5                    & 92.8                   & 0.7   \\
% \bottomrule
% \end{tabular}
% % Uncomment for resize
% }
% \caption{Performance of \alignedmlm{} when varying the percentage of tokens in the bilingual dictionary between \lang1 and \lang2.}
% \end{table*}

==> LaTeX/001_checklist.tex <==
\section*{To Do}

\begin{enumerate}
    \item \sout{Abstract - \ameet{}}
    \item \sout{Introduction - \ameet{}}
    \item \sout{Related work - \ameet{}}
    \item Approach - \ameet{}
    \begin{enumerate}
        \item Figure - \ameet{}
        \item \sout{Evaluation - \ameet{}}
    \end{enumerate}
    \item Experimental setup - \henry{}
    \item Results - \ameet{} \henry{}
    \begin{enumerate}
        \item Bar plots - \henry{}
        \item Tables - \henry{}
    \end{enumerate}    
    \item Conclusion
    \item Appendix
\end{enumerate}
